TheanoLM - An Extensible Toolkit for Neural Network Language Modeling

We present a new tool for training neural network language models (NNLMs), scoring sentences, and generating text. The tool has been written using Python library Theano, which allows researcher to easily extend it and tune any aspect of the training process. Regardless of the flexibility, Theano is able to generate extremely fast native code that can utilize a GPU or multiple CPU cores in order to parallelize the heavy numerical computations. The tool has been evaluated in difficult Finnish and English conversational speech recognition tasks, and significant improvement was obtained over our best back-off n-gram models. The results that we obtained in the Finnish task were compared to those from existing RNNLM and RWTHLM toolkits, and found to be as good or better, while training times were an order of magnitude shorter.

==> tcblistings.code.tex <==
%% The LaTeX package tcolorbox - version 2.70 (2014/02/06)
%% tcblistings.code.tex: Code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2014 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{2.70}

\RequirePackage{listings}[2007/02/22]

\tcbuselibrary{listings@core}

\let\tcb@listing@MakeCaption@org=\lst@MakeCaption

\def\tcb@listing@set@MakeCaption@org{%
  \let\lst@MakeCaption\tcb@listing@MakeCaption@org}
\def\tcb@listing@set@MakeCaption@empty{%
  \lst@HRefStepCounter{lstlisting}%
  \let\lst@MakeCaption\@gobble}

\lstdefinestyle{tcblatex}{language={[LaTeX]TeX},
     aboveskip={0\p@ \@plus 6\p@}, belowskip={0\p@ \@plus 6\p@},
     columns=fullflexible, keepspaces=true,
     breaklines=true, breakatwhitespace=true,
     basicstyle=\ttfamily\small, extendedchars=true, nolol,
     inputencoding=\kvtcb@listingencoding}

\def\tcb@listing@input@listing#1#2{%
  \begingroup%
  \toks@=\expandafter{#1}%
  \edef\tcb@temp{\noexpand\lstinputlisting[nolol,\the\toks@]}%
  \tcb@listing@set@MakeCaption%
  \tcb@temp{#2}%
  \endgroup%
}%


\def\tcb@listing@uselistinglisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@listingfile}%
}%

\def\tcb@listing@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@listingoptions}{\kvtcb@tempfile}%
}%

\def\tcb@listing@doc@usetemplisting{%
  \tcb@listing@input@listing{\kvtcb@doclistingoptions}{\kvtcb@tempfile}%
}

\tcbset{%
  listing options/.store in=\kvtcb@listingoptions,%
  listing style/.style={listing options={style=#1}},%
  no listing options/.style={listing options=},%
  listing inputencoding/.store in=\kvtcb@listingencoding,%
  listing remove caption/.is choice,
  listing remove caption/true/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@empty},
  listing remove caption/false/.code={\let\tcb@listing@set@MakeCaption\tcb@listing@set@MakeCaption@org},
  listing remove caption/.default=true,
  listing engine/listings/.code={\let\tcbuselistinglisting\tcb@listing@uselistinglisting%
    \let\tcbusetemplisting\tcb@listing@usetemplisting%
    \let\tcb@doc@usetemplisting\tcb@listing@doc@usetemplisting},
}


\tcbset{%
  reset@listings/.style={%
    listing style=tcblatex,
    listing inputencoding=\inputencodingname,
    listing remove caption,
    listing engine=listings,
  },
  initialize@reset=reset@listings,
}



==> tcblistingscore.code.tex <==
%% The LaTeX package tcolorbox - version 2.70 (2014/02/06)
%% tcblistingscode.code.tex: Auxiliary code for colorboxes with listings
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2014 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{2.70}

\def\tcbuselistingtext{\input{\kvtcb@listingfile}}%

\def\tcb@listing@listingAndText{%
   \tcbuselistinglisting%
   \tcblower%
   \tcbuselistingtext%
}

\def\tcb@listing@listingAndComment{%
   \tcbuselistinglisting%
   \tcblower%
   \kvtcb@listingcomment%
}

\def\tcb@listing@textAndListing{%
   \tcbuselistingtext%
   \tcblower%
   \tcbuselistinglisting%
}

\def\tcb@listing@commentAndListing{%
   \kvtcb@listingcomment%
   \tcblower%
   \tcbuselistinglisting%
}

\def\tcb@listing@listing{%
  \tcbuselistinglisting%
}

\def\tcb@inputlisting@out@textAboveListing{%
  \kvtcb@beforebox\noindent%
  \iftcb@lowervisible\tcb@minipage{\kvtcb@width}\color{\kvtcb@collower}\kvtcb@fontlower\kvtcb@before@lower\ignorespaces%
     \begingroup\tcb@layer@inc\tcbuselistingtext\tcb@layer@dec\endgroup%
     \unskip\kvtcb@after@lower\endminipage%
     \par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
     \fi%
  \begin{tcolorbox}[before=]\tcbuselistinglisting\end{tcolorbox}%
}

\def\tcb@inputlisting@out@listingAboveText{%
  \begin{tcolorbox}[after=]\tcbuselistinglisting\end{tcolorbox}%
  \iftcb@lowervisible\par\vskip-\parskip\vspace*{\kvtcb@middle}\noindent%
    \tcb@minipage{\kvtcb@width}\color{\kvtcb@collower}\kvtcb@fontlower\kvtcb@before@lower\ignorespaces%
     \begingroup\tcb@layer@inc\tcbuselistingtext\tcb@layer@dec\endgroup%
     \unskip\kvtcb@after@lower\endminipage\fi%
  \kvtcb@afterbox%
}

\def\tcb@inputlisting@out@prepare{%
  \tcbdimto\tcb@width{\kvtcb@width}%
  \tcbdimto\tcb@innerwidth{\tcb@width-\kvtcb@left@rule-\kvtcb@right@rule}%
  \tcbdimto\tcb@temp{\tcb@innerwidth-\kvtcb@boxsep*2}%
  \tcbdimto\tcb@w@upper{\tcb@temp-\kvtcb@leftupper-\kvtcb@rightupper}%
  \tcbset{breakable@false}%
  \def\tcb@minipage{\csname tcb@minipage@\kvtcb@sbs@align\endcsname}%
  \tcbdimto\tcb@w@upper@real{\tcb@w@upper}%
  \tcbdimto\tcb@w@sbs{\tcb@w@upper@real-\kvtcb@sbs@gap}%
  \tcb@sbs@quota%
  \ifx\kvtcb@float\@empty%
    \newenvironment{tcb@sbsfloat}{\kvtcb@beforebox}{\kvtcb@afterbox}%
  \else%
    \edef\float@start{\noexpand\@float{tcbfloat}[\kvtcb@float]}%
    \newenvironment{tcb@sbsfloat}{\float@start}{\end@float}%
  \fi%
}

\def\tcb@inputlisting@out@listingAndText{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@lower}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@lower-\kvtcb@sbs@gap}%
  \begin{tcb@sbsfloat}\begin{minipage}{\tcb@width}%
  \tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage\hfill%
  \iftcb@lowervisible\tcb@minipage{\tcb@w@outside}\color{\kvtcb@collower}\kvtcb@fontlower\kvtcb@before@lower\ignorespaces%
    \begingroup\tcb@layer@inc\tcbuselistingtext\tcb@layer@dec\endgroup%
    \unskip\kvtcb@after@lower\endminipage\fi%
  \end{minipage}\end{tcb@sbsfloat}%
}

\def\tcb@inputlisting@out@textAndListing{%
  \tcb@inputlisting@out@prepare%
  \tcbdimto\tcb@w@outside{\tcb@w@upper}%
  \tcbdimto\tcb@w@inside{\tcb@width-\tcb@w@upper-\kvtcb@sbs@gap}%
  \begin{tcb@sbsfloat}\begin{minipage}{\tcb@width}%
  \iftcb@lowervisible\tcb@minipage{\tcb@w@outside}\color{\kvtcb@collower}\kvtcb@fontlower\kvtcb@before@lower\ignorespaces%
    \begingroup\tcb@layer@inc\tcbuselistingtext\tcb@layer@dec\endgroup%
    \unskip\kvtcb@after@lower\endminipage\fi\hfill%
  \tcb@minipage{\tcb@w@inside}%
  \begin{tcolorbox}[width=\tcb@w@inside,nobeforeafter,nofloat,sidebyside=false]\tcbuselistinglisting\end{tcolorbox}%
  \endminipage%
  \end{minipage}\end{tcb@sbsfloat}%
}

\def\tcb@inputlisting@inside{%
  \begin{tcolorbox}[capture=\tcb@listing@capture]\tcb@listing@process\end{tcolorbox}%
}

\let\tcb@inputlisting\tcb@inputlisting@inside

\def\tcb@set@listing@process#1{%
  \let\tcb@inputlisting\tcb@inputlisting@inside%
  \let\tcb@listing@process=#1%
}

\tcbset{%
  listing file/.store in=\kvtcb@listingfile,%
  comment/.store in=\kvtcb@listingcomment,%
  listing and text/.code={\tcb@set@listing@process{\tcb@listing@listingAndText}},%
  text and listing/.code={\tcb@set@listing@process{\tcb@listing@textAndListing}},%
  listing and comment/.code={\tcb@set@listing@process{\tcb@listing@listingAndComment}},%
  comment and listing/.code={\tcb@set@listing@process{\tcb@listing@commentAndListing}},%
  listing only/.code={\tcb@set@listing@process{\tcb@listing@listing}},%
  text only/.code={\tcb@set@listing@process{\tcbuselistingtext}},%
  text above listing/.code={\let\tcb@inputlisting\tcb@inputlisting@out@textAboveListing},%
  listing above text/.code={\let\tcb@inputlisting\tcb@inputlisting@out@listingAboveText},%
  text side listing/.style={sidebyside,text and listing},%
  listing side text/.style={sidebyside,listing and text},%
  text outside listing/.code={\let\tcb@inputlisting\tcb@inputlisting@out@textAndListing},%
  listing outside text/.code={\let\tcb@inputlisting\tcb@inputlisting@out@listingAndText},%
  listing engine/.is choice,
}

\newenvironment{tcblisting}[1]{%
  \def\tcblisting@box{\tcbinputlisting{#1}}%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup%
  \tcblisting@box%
}

\long\def\tcbinputlisting#1{%
  \begingroup%
  \tcb@layer@pushup%
  \tcbset{capture=minipage,#1}\tcb@afteroptions@hook%
  \let\tcb@listing@capture=\kvtcb@capture%
  \tcb@inputlisting\endgroup%
}

\newenvironment{tcboutputlisting}{%
  \begingroup\tcbverbatimwrite{\kvtcb@listingfile}%
}{\endtcbverbatimwrite\endgroup}


\long\def\tcb@newtcblisting#1#2{\tcb@newenvironment{#1}{\tcblisting{#2,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@#1[#2]#3{\tcb@newenvironment{#1}[#2]{\tcblisting{#3,options@for=#1}}{\endtcblisting}}

\long\def\tcb@newtcblisting@@#1[#2][#3]#4{\tcb@newenvironment{#1}[#2][#3]{\tcblisting{#4,options@for=#1}}{\endtcblisting}}

\long\def\tcb@new@tcblisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcblisting@@{#1}[#2]}{\tcb@newtcblisting@{#1}[#2]}}

\long\def\tcb@new@tcblisting#1{%
  \preto\tcb@new@colopt{savedelimiter=#1}%
  \cslet{tcb@opt@#1}{\tcb@new@colopt}%
  \@ifnextchar[{\tcb@new@tcblisting@{#1}}{\tcb@newtcblisting{#1}}}

\long\def\tcb@new@tcblisting@opt[#1]#2{%
  \tcb@proc@options@init{#1}{#2}%
  \tcb@new@tcblisting{#2}%
}

\long\def\new@tcblisting{%
  \def\tcb@new@colopt{}%
  \@ifnextchar[{\tcb@new@tcblisting@opt}{\tcb@new@tcblisting}}

\long\def\newtcblisting{%
  \let\tcb@newenvironment\newenvironment%
  \new@tcblisting}

\long\def\renewtcblisting{%
  \let\tcb@newenvironment\renewenvironment%
  \new@tcblisting}

\long\def\tcb@newtcbinputlisting#1#2{\expandafter\tcb@newcommand\csname#1\endcsname{\tcbinputlisting{#2,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@#1[#2]#3{\expandafter\tcb@newcommand\csname#1\endcsname[#2]{\tcbinputlisting{#3,options@for=#1}}}

\long\def\tcb@newtcbinputlisting@@#1[#2][#3]#4{\expandafter\tcb@newcommand\csname#1\endcsname[#2][#3]{\tcbinputlisting{#4,options@for=#1}}}

\long\def\tcb@new@tcbinputlisting@#1[#2]{%
  \@ifnextchar[{\tcb@newtcbinputlisting@@{#1}[#2]}{\tcb@newtcbinputlisting@{#1}[#2]}}

\long\def\tcb@new@tcbinputlisting#1{%
  \preto\tcb@new@colopt{savedelimiter=#1}%
  \cslet{tcb@opt@#1}{\tcb@new@colopt}%
  \@ifnextchar[{\tcb@new@tcbinputlisting@{#1}}{\tcb@newtcbinputlisting{#1}}}


\long\def\tcb@new@tcbinputlisting@bs#1{%
  \edef\tcb@temp{\noexpand\tcb@new@tcbinputlisting{\tcb@remove@bs{#1}}}%
  \tcb@temp%
}

\long\def\tcb@new@tcbinputlisting@opt#1#2{%
  \tcb@proc@options@init{#2}{#1}%
  \tcb@new@tcbinputlisting{#1}%
}

\long\def\tcb@new@tcbinputlisting@opt@bs[#1]#2{%
  \edef\tcb@temp{\noexpand\tcb@new@tcbinputlisting@opt{\tcb@remove@bs{#2}}}%
  \tcb@temp{#1}%
}

\long\def\new@tcbinputlisting{%
  \def\tcb@new@colopt{}%
  \@ifnextchar[{\tcb@new@tcbinputlisting@opt@bs}{\tcb@new@tcbinputlisting@bs}}

\long\def\newtcbinputlisting{%
  \let\tcb@newcommand\newcommand%
  \new@tcbinputlisting}

\long\def\renewtcbinputlisting{%
  \let\tcb@newcommand\renewcommand%
  \new@tcbinputlisting}


\tcbset{%
  reset@listingscore/.style={%
    listing file=\jobname.listing,
    comment=,
    listing and text,
  },
  initialize@reset=reset@listingscore,
}


